CoSTL: Comprehensive Spatial-Temporal Representation Learning for Moment Retrieval and Highlight Detection

Video Moment Retrieval (MR) and Highlight Detection (HD) are crucial tasks in video analysis that aim to localize specific moments and estimate clip-wise relevance based on a given text query. Recent approaches treat them as similar video grounding tasks and use the same architecture to solve them. These tasks require both fine-grained comprehension at the image level and high-level temporal understanding across the entire video. Existing approaches have primarily focused on temporal modeling using frame-level features, often neglecting the rich visual information related to the text query within individual frames. This oversight leads to inaccurate grounding results. To address this limitation, we propose a Comprehensive Spatial-Temporal Representation Learning Framework (CoSTL), which captures both fine-grained image-level information and temporal dynamics. Specifically, CoSTL incorporates a text-driven progressive fine-grained image encoder, performing a two-step text-driven knowledge extraction process to learn fine-grained spatial representations. Furthermore, a multi-scale temporal perception module captures comprehensive spatial-temporal representations, enhancing the model's ability to process temporal dynamics. We demonstrate state-of-the-art performance on four public benchmarks: QVHighlights, Charades-STA, TACoS, and TVSum.

==> 3_tab/1_qvhl_copy.tex <==
\begin{table*}[h]
    \centering

    % \caption{Video moment retrieval (MR) and highlight detection (HD) results on QVHighlights test split. 
    % \protect\tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); denotes CLIP\_B/32, \\
    % \protect\tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); denotes SlowFast R-50, \protect\tikz\draw[fill={rgb:yellow,1;white,2}, draw=black] (0,0) circle (0.1cm); denotes audio features and
    % \protect\tikz\draw[fill={rgb:red,1;white,2}, draw=black] (0,0) circle (0.1cm); denotes BLIP2 (CLIP\_L) feature. The best and second-best metrics are marked with \textbf{bold} and \underline{underline}, respectively.}
    
    \caption{Video moment retrieval (MR) and highlight detection (HD) results on QVHighlights test split. 
    \protect\tikz[baseline]{\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm);} denotes CLIP\_B/32, \\
    \protect\tikz[baseline]{\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm);} denotes SlowFast R-50, \protect\tikz[baseline]{\draw[fill={rgb:yellow,1;white,2}, draw=black] (0,0) circle (0.1cm);} denotes audio features and
    \protect\tikz[baseline]{\draw[fill={rgb:red,1;white,2}, draw=black] (0,0) circle (0.1cm);} denotes BLIP2 (CLIP\_L) feature. The best and second-best metrics are marked with \textbf{bold} and \underline{underline}, respectively.}


    \begin{tabular}{cccccccccc}
        \toprule
        \multirow{3}{*}{Method} & \multirow{3}{*}{Backbone} & \multirow{3}{*}{Pretrain} & \multicolumn{5}{c}{MR} & \multicolumn{2}{c}{HD} \\ \cmidrule(lr){4-8} \cmidrule(lr){9-10}
        & & & \multicolumn{2}{c}{R1} & \multicolumn{3}{c}{mAP} & \multicolumn{2}{c}{$\geq$ Very Good} \\ \cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10}
        & & & @0.5 & @0.7 & @0.5 & @0.75 & Avg. & mAP & HIT@1  \\ \midrule
        M-DETR\cite{mdetr} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 52.89 & 33.02 & 54.82 & 29.40 & 30.73 & 35.69 & 20.88 \\
          UniVTG\cite{univtg} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 58.86 & 40.86 & 57.60 & 35.59& 35.47 & 38.20 & 60.96 \\ 
          MH-DETR\cite{mhdetr} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 60.05 & 42.48 & 60.75 & 38.18 & 38.38 & 38.22 & 60.51 \\ 
          EaTR\cite{eatr} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 61.36 &45.79& 61.86& 41.91& 41.74& 37.15& 58.65  \\ 
        QD-DETR\cite{qddetr} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 62.40 & 44.96 & 62.52 & 39.88 & 39.86 & 38.94 & 62.40 \\
        CG-DETR\cite{cgdetr} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 65.43& 48.38& 64.51& 42.77& 42.86& 40.33& 66.21 \\
        UVCOM\cite{uvcom} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 63.55 & 47.47 & 63.37 & 42.67 & 43.18 & 39.74 & 64.20 \\ 
        UVCOM\textsuperscript{*}\cite{uvcom} & \tikz\draw[fill={rgb:red,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & \underline{68.52} & \underline{51.94} & 65.40 & 44.06 & 43.78 & 40.64 & 65.42 \\ 
        R2-tuning\cite{uvcom} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & 68.03 & 49.35 & \underline{69.04} & \underline{47.56} & \underline{46.17} & \underline{40.75} & 64.20 \\
        \midrule
        UMT\cite{umt} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:yellow,1;white,2}, draw=black] (0,0) circle (0.1cm);& \checkmark & 60.83 & 43.26 & 57.33 & 39.12 & 38.08 & 39.12 & 62.39 \\ 
          UniVTG\cite{univtg} & \tikz\draw[fill={rgb:blue,1;white,2}, draw=black] (0,0) circle (0.1cm); \tikz\draw[fill={rgb:green,1;white,2}, draw=black] (0,0) circle (0.1cm); & \checkmark & 65.43 & 50.06 & 64.06 & 45.02& 43.63 & 40.54 & \underline{66.28} \\ 
        \midrule
        \textbf{CoSTL (Ours)} & \tikz\draw[fill={rgb:red,1;white,2}, draw=black] (0,0) circle (0.1cm); & \ding{55} & \textbf{75.43} & \textbf{54.24} & \textbf{71.48} & \textbf{48.45} & \textbf{46.68} & \textbf{41.36} & \textbf{71.59} \\
        \bottomrule
    \end{tabular}
    \label{tab:qvhighlight}
\end{table*}

